Context-Based Tweet Engagement Prediction

Twitter is currently one of the biggest social media platforms. Its users may share, read, and engage with short posts called tweets. For the ACM Recommender Systems Conference 2020, Twitter published a dataset around 70 GB in size for the annual RecSys Challenge. In 2020, the RecSys Challenge invited participating teams to create models that would predict engagement likelihoods for given user-tweet combinations. The submitted models predicting like, reply, retweet, and quote engagements were evaluated based on two metrics: area under the precision-recall curve (PRAUC) and relative cross-entropy (RCE). In this diploma thesis, we used the RecSys 2020 Challenge dataset and evaluation procedure to investigate how well context alone may be used to predict tweet engagement likelihood. In doing so, we employed the Spark engine on TU Wien's Little Big Data Cluster to create scalable data preprocessing, feature engineering, feature selection, and machine learning pipelines. We manually created just under 200 additional features to describe tweet context. The results indicate that features describing users' prior engagement history and the popularity of hashtags and links in the tweet were the most informative. We also found that factors such as the prediction algorithm, training dataset size, training dataset sampling method, and feature selection significantly affect the results. After comparing the best results of our context-only prediction models with content-only models and with models developed by the Challenge winners, we identified that the context-based models underperformed in terms of the RCE score. This work thus concludes by situating this discrepancy and proposing potential improvements to our implementation, which is shared in a public git repository.

==> Lists/finalDFsDash.tex <==
-- 747M    Final\_ test\_ EU\_ sample\_ 10pct.parquet \\
-- 76M     Final\_ test\_ EU\_ sample\_ 1pct.parquet \\
-- 146M    Final\_ test\_ EU\_ sample\_ 2pct.parquet \\
-- 369M    Final\_ test\_ EU\_ sample\_ 5pct.parquet \\
-- 423M    Final\_ test\_ EWU\_ sample\_ 10pct.parquet \\
-- 55M     Final\_ test\_ EWU\_ sample\_ 1pct.parquet \\
-- 105M    Final\_ test\_ EWU\_ sample\_ 2pct.parquet \\
-- 261M    Final\_ test\_ EWU\_ sample\_ 5pct.parquet \\
-- 616M    Final\_ test\_ inter\_ EWU+EU\_ sample\_ 10pct.parquet \\
-- 64M     Final\_ test\_ inter\_ EWU+EU\_ sample\_ 1pct.parquet \\
-- 118M    Final\_ test\_ inter\_ EWU+EU\_ sample\_ 2pct.parquet \\
-- 290M    Final\_ test\_ inter\_ EWU+EU\_ sample\_ 5pct.parquet \\
-- 7.8G    Final\_ test.parquet \\
-- 750M    Final\_ test\_ random\_ sample\_ 10pct.parquet \\
-- 76M     Final\_ test\_ random\_ sample\_ 1pct.parquet \\
-- 145M    Final\_ test\_ random\_ sample\_ 2pct.parquet \\
-- 368M    Final\_ test\_ random\_ sample\_ 5pct.parquet \\
-- 706M    Final\_ test\_ tweet\_ sample\_ 10pct.parquet \\
-- 69M     Final\_ test\_ tweet\_ sample\_ 1pct.parquet \\
-- 131M    Final\_ test\_ tweet\_ sample\_ 2pct.parquet \\
-- 340M    Final\_ test\_ tweet\_ sample\_ 5pct.parquet \\
-- 4.8G    Final\_ train\_ EU\_ sample\_ 10pct.parquet \\
-- 464M    Final\_ train\_ EU\_ sample\_ 1pct.parquet \\
-- 939M    Final\_ train\_ EU\_ sample\_ 2pct.parquet \\
-- 2.4G    Final\_ train\_ EU\_ sample\_ 5pct.parquet \\
-- 4.0G    Final\_ train\_ EWU\_ sample\_ 10pct.parquet \\
-- 480M    Final\_ train\_ EWU\_ sample\_ 1pct.parquet \\
-- 922M    Final\_ train\_ EWU\_ sample\_ 2pct.parquet \\
-- 2.3G    Final\_ train\_ EWU\_ sample\_ 5pct.parquet \\
-- 4.7G    Final\_ train\_ inter\_ EWU+EU\_ sample\_ 10pct.parquet \\
-- 480M    Final\_ train\_ inter\_ EWU+EU\_ sample\_ 1pct.parquet \\
-- 973M    Final\_ train\_ inter\_ EWU+EU\_ sample\_ 2pct.parquet \\
-- 2.4G    Final\_ train\_ inter\_ EWU+EU\_ sample\_ 5pct.parquet \\
-- 53G     Final\_ train.parquet \\
-- 4.7G    Final\_ train\_ random\_ sample\_ 10pct.parquet \\
-- 447M    Final\_ train\_ random\_ sample\_ 1pct.parquet \\
-- 906M    Final\_ train\_ random\_ sample\_ 2pct.parquet \\
-- 2.3G    Final\_ train\_ random\_ sample\_ 5pct.parquet \\
-- 4.3G    Final\_ train\_ tweet\_ sample\_ 10pct.parquet \\
-- 384M    Final\_ train\_ tweet\_ sample\_ 1pct.parquet \\
-- 794M    Final\_ train\_ tweet\_ sample\_ 2pct.parquet \\
-- 242M    Final\_ train\_ tweet\_ sample\_ 5pct.parquet \\
-- 743M    Final\_ val\_ EU\_ sample\_ 10pct.parquet \\
-- 75M     Final\_ val\_ EU\_ sample\_ 1pct.parquet \\
-- 145M    Final\_ val\_ EU\_ sample\_ 2pct.parquet \\
-- 365M    Final\_ val\_ EU\_ sample\_ 5pct.parquet \\
-- 540M    Final\_ val\_ EWU\_ sample\_ 10pct.parquet \\
-- 58M     Final\_ val\_ EWU\_ sample\_ 1pct.parquet \\
-- 109M    Final\_ val\_ EWU\_ sample\_ 2pct.parquet \\
-- 262M    Final\_ val\_ EWU\_ sample\_ 5pct.parquet \\
-- 608M    Final\_ val\_ inter\_ EWU+EU\_ sample\_ 10pct.parquet \\
-- 64M     Final\_ val\_ inter\_ EWU+EU\_ sample\_ 1pct.parquet \\
-- 117M    Final\_ val\_ inter\_ EWU+EU\_ sample\_ 2pct.parquet \\
-- 286M    Final\_ val\_ inter\_ EWU+EU\_ sample\_ 5pct.parquet \\
-- 7.7G    Final\_ val.parquet \\
-- 745M    Final\_ val\_ random\_ sample\_ 10pct.parquet \\
-- 75M     Final\_ val\_ random\_ sample\_ 1pct.parquet \\
-- 145M    Final\_ val\_ random\_ sample\_ 2pct.parquet \\
-- 366M    Final\_ val\_ random\_ sample\_ 5pct.parquet \\
-- 1.4G    Final\_ val+test\_ EU\_ sample\_ 10pct.parquet \\
-- 137M    Final\_ val+test\_ EU\_ sample\_ 1pct.parquet \\
-- 277M    Final\_ val+test\_ EU\_ sample\_ 2pct.parquet \\
-- 704M    Final\_ val+test\_ EU\_ sample\_ 5pct.parquet \\
-- 899M    Final\_ val+test\_ EWU\_ sample\_ 10pct.parquet \\
-- 101M    Final\_ val+test\_ EWU\_ sample\_ 1pct.parquet \\
-- 201M    Final\_ val+test\_ EWU\_ sample\_ 2pct.parquet \\
-- 509M    Final\_ val+test\_ EWU\_ sample\_ 5pct.parquet \\
-- 1.2G    Final\_ val+test\_ inter\_ EWU+EU\_ sample\_ 10pct.parquet \\
-- 114M    Final\_ val+test\_ inter\_ EWU+EU\_ sample\_ 1pct.parquet \\
-- 142M    Final\_ val+test\_ inter\_ EWU+EU\_ sample\_ 2pct.parquet \\
-- 652M    Final\_ val+test\_ inter\_ EWU+EU\_ sample\_ 5pct.parquet \\
-- 16G     Final\_ val+test.parquet \\
-- 1.5G    Final\_ val+test\_ random\_ sample\_ 10pct.parquet \\
-- 137M    Final\_ val+test\_ random\_ sample\_ 1pct.parquet \\
-- 277M    Final\_ val+test\_ random\_ sample\_ 2pct.parquet \\
-- 705M    Final\_ val+test\_ random\_ sample\_ 5pct.parquet \\
-- 1.4G    Final\_ val+test\_ tweet\_ sample\_ 10pct.parquet \\
-- 123M    Final\_ val+test\_ tweet\_ sample\_ 1pct.parquet \\
-- 248M    Final\_ val+test\_ tweet\_ sample\_ 2pct.parquet \\
-- 654M    Final\_ val+test\_ tweet\_ sample\_ 5pct.parquet \\
-- 701M    Final\_ val\_ tweet\_ sample\_ 10pct.parquet \\
-- 69M     Final\_ val\_ tweet\_ sample\_ 1pct.parquet \\
-- 130M    Final\_ val\_ tweet\_ sample\_ 2pct.parquet \\
-- 339M    Final\_ val\_ tweet\_ sample\_ 5pct.parquet

==> Tables/EvalValueCounts/final_deflattened_PRAUC-algorithm-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of algorithm in final_deflattened_PRAUC}
\label{tabfinal_deflattened_PRAUCalgorithm}\\
\toprule
 algorithm \\
\midrule
\endfirsthead
\caption[]{Counts of values of algorithm in final_deflattened_PRAUC} \\
\toprule
 algorithm \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
      4152 \\
      3771 \\
      2062 \\
      1707 \\
       174 \\
        73 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_PRAUC-eo_dataset-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of eo_dataset in final_deflattened_PRAUC}
\label{tabfinal_deflattened_PRAUCeo_dataset}\\
\toprule
 eo\_dataset \\
\midrule
\endfirsthead
\caption[]{Counts of values of eo_dataset in final_deflattened_PRAUC} \\
\toprule
 eo\_dataset \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       3870 \\
       3849 \\
       3804 \\
        416 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_PRAUC-eo_percent-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of eo_percent in final_deflattened_PRAUC}
\label{tabfinal_deflattened_PRAUCeo_percent}\\
\toprule
 eo\_percent \\
\midrule
\endfirsthead
\caption[]{Counts of values of eo_percent in final_deflattened_PRAUC} \\
\toprule
 eo\_percent \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       6583 \\
       2234 \\
       1591 \\
       1336 \\
        195 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_PRAUC-eo_technique-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of eo_technique in final_deflattened_PRAUC}
\label{tabfinal_deflattened_PRAUCeo_technique}\\
\toprule
 eo\_technique \\
\midrule
\endfirsthead
\caption[]{Counts of values of eo_technique in final_deflattened_PRAUC} \\
\toprule
 eo\_technique \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
         2752 \\
         2272 \\
         2264 \\
         2263 \\
         2193 \\
          195 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_PRAUC-evaluated_on-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of evaluated_on in final_deflattened_PRAUC}
\label{tabfinal_deflattened_PRAUCevaluated_on}\\
\toprule
 evaluated\_on \\
\midrule
\endfirsthead
\caption[]{Counts of values of evaluated_on in final_deflattened_PRAUC} \\
\toprule
 evaluated\_on \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
          479 \\
          473 \\
          455 \\
          427 \\
          425 \\
          425 \\
          424 \\
          424 \\
          424 \\
          420 \\
          418 \\
          417 \\
          417 \\
          413 \\
          413 \\
          213 \\
          213 \\
          213 \\
          127 \\
          127 \\
          127 \\
          127 \\
          127 \\
          126 \\
          123 \\
          123 \\
          123 \\
          123 \\
          118 \\
          118 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
           98 \\
           97 \\
           97 \\
           97 \\
           97 \\
           97 \\
           97 \\
           88 \\
           88 \\
           86 \\
           81 \\
           81 \\
           81 \\
           78 \\
           78 \\
           78 \\
           72 \\
           72 \\
           72 \\
           65 \\
           65 \\
           65 \\
           40 \\
           25 \\
           23 \\
           23 \\
           23 \\
           21 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           16 \\
           15 \\
           15 \\
           15 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_PRAUC-feature_selection-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of feature_selection in final\_deflattened\_PRAUC}
\label{tabfinal_deflattened_PRAUCfeature_selection}\\
\toprule
 feature\_selection \\
\midrule
\endfirsthead
\caption[]{Counts of values of feature_selection in final\_deflattened\_PRAUC} \\
\toprule
 feature\_selection \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
              4600 \\
              1987 \\
              1814 \\
              1802 \\
              1736 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_PRAUC-note-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of note in final_deflattened_PRAUC}
\label{tabfinal_deflattened_PRAUCnote}\\
\toprule
 note \\
\midrule
\endfirsthead
\caption[]{Counts of values of note in final_deflattened_PRAUC} \\
\toprule
 note \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
11308 \\
  631 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_PRAUC-to_dataset-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of to_dataset in final_deflattened_PRAUC}
\label{tabfinal_deflattened_PRAUCto_dataset}\\
\toprule
 to\_dataset \\
\midrule
\endfirsthead
\caption[]{Counts of values of to_dataset in final_deflattened_PRAUC} \\
\toprule
 to\_dataset \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       7661 \\
       2498 \\
       1058 \\
        722 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_PRAUC-to_percent-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of to_percent in final_deflattened_PRAUC}
\label{tabfinal_deflattened_PRAUCto_percent}\\
\toprule
 to\_percent \\
\midrule
\endfirsthead
\caption[]{Counts of values of to_percent in final_deflattened_PRAUC} \\
\toprule
 to\_percent \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       5128 \\
       4022 \\
       1606 \\
       1183 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_PRAUC-algorithm-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of algorithm in final_deflattened_nonan_PRAUC}
\label{tabfinal_deflattened_nonan_PRAUCalgorithm}\\
\toprule
 algorithm \\
\midrule
\endfirsthead
\caption[]{Counts of values of algorithm in final_deflattened_nonan_PRAUC} \\
\toprule
 algorithm \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
      4152 \\
      3771 \\
      2062 \\
      1707 \\
       174 \\
        73 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_PRAUC-eo_dataset-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of eo_dataset in final_deflattened_nonan_PRAUC}
\label{tabfinal_deflattened_nonan_PRAUCeo_dataset}\\
\toprule
 eo\_dataset \\
\midrule
\endfirsthead
\caption[]{Counts of values of eo_dataset in final_deflattened_nonan_PRAUC} \\
\toprule
 eo\_dataset \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       3870 \\
       3849 \\
       3804 \\
        416 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_PRAUC-eo_percent-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of eo_percent in final_deflattened_nonan_PRAUC}
\label{tabfinal_deflattened_nonan_PRAUCeo_percent}\\
\toprule
 eo\_percent \\
\midrule
\endfirsthead
\caption[]{Counts of values of eo_percent in final_deflattened_nonan_PRAUC} \\
\toprule
 eo\_percent \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       6583 \\
       2234 \\
       1591 \\
       1336 \\
        195 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_PRAUC-eo_technique-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of eo_technique in final_deflattened_nonan_PRAUC}
\label{tabfinal_deflattened_nonan_PRAUCeo_technique}\\
\toprule
 eo\_technique \\
\midrule
\endfirsthead
\caption[]{Counts of values of eo_technique in final_deflattened_nonan_PRAUC} \\
\toprule
 eo\_technique \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
         2752 \\
         2272 \\
         2264 \\
         2263 \\
         2193 \\
          195 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_PRAUC-evaluated_on-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of evaluated_on in final_deflattened_nonan_PRAUC}
\label{tabfinal_deflattened_nonan_PRAUCevaluated_on}\\
\toprule
 evaluated\_on \\
\midrule
\endfirsthead
\caption[]{Counts of values of evaluated_on in final_deflattened_nonan_PRAUC} \\
\toprule
 evaluated\_on \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
          479 \\
          473 \\
          455 \\
          427 \\
          425 \\
          425 \\
          424 \\
          424 \\
          424 \\
          420 \\
          418 \\
          417 \\
          417 \\
          413 \\
          413 \\
          213 \\
          213 \\
          213 \\
          127 \\
          127 \\
          127 \\
          127 \\
          127 \\
          126 \\
          123 \\
          123 \\
          123 \\
          123 \\
          118 \\
          118 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
           98 \\
           97 \\
           97 \\
           97 \\
           97 \\
           97 \\
           97 \\
           88 \\
           88 \\
           86 \\
           81 \\
           81 \\
           81 \\
           78 \\
           78 \\
           78 \\
           72 \\
           72 \\
           72 \\
           65 \\
           65 \\
           65 \\
           40 \\
           25 \\
           23 \\
           23 \\
           23 \\
           21 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           16 \\
           15 \\
           15 \\
           15 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_PRAUC-feature_selection-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of feature_selection in final_deflattened_nonan_PRAUC}
\label{tabfinal_deflattened_nonan_PRAUCfeature_selection}\\
\toprule
 feature\_selection \\
\midrule
\endfirsthead
\caption[]{Counts of values of feature_selection in final_deflattened_nonan_PRAUC} \\
\toprule
 feature\_selection \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
              4600 \\
              1987 \\
              1814 \\
              1802 \\
              1736 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_PRAUC-note-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of note in final_deflattened_nonan_PRAUC}
\label{tabfinal_deflattened_nonan_PRAUCnote}\\
\toprule
 note \\
\midrule
\endfirsthead
\caption[]{Counts of values of note in final_deflattened_nonan_PRAUC} \\
\toprule
 note \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
11308 \\
  631 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_PRAUC-to_dataset-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of to_dataset in final_deflattened_nonan_PRAUC}
\label{tabfinal_deflattened_nonan_PRAUCto_dataset}\\
\toprule
 to\_dataset \\
\midrule
\endfirsthead
\caption[]{Counts of values of to_dataset in final_deflattened_nonan_PRAUC} \\
\toprule
 to\_dataset \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       7661 \\
       2498 \\
       1058 \\
        722 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_PRAUC-to_percent-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of to_percent in final_deflattened_nonan_PRAUC}
\label{tabfinal_deflattened_nonan_PRAUCto_percent}\\
\toprule
 to\_percent \\
\midrule
\endfirsthead
\caption[]{Counts of values of to_percent in final_deflattened_nonan_PRAUC} \\
\toprule
 to\_percent \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       5128 \\
       4022 \\
       1606 \\
       1183 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_PRAUC-to_technique-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of to_technique in final_deflattened_nonan_PRAUC}
\label{tabfinal_deflattened_nonan_PRAUCto_technique}\\
\toprule
 to\_technique \\
\midrule
\endfirsthead
\caption[]{Counts of values of to_technique in final_deflattened_nonan_PRAUC} \\
\toprule
 to\_technique \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
         3885 \\
         2413 \\
         2353 \\
         2123 \\
         1165 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_PRAUC-trained_on-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of trained_on in final_deflattened_nonan_PRAUC}
\label{tabfinal_deflattened_nonan_PRAUCtrained_on}\\
\toprule
 trained\_on \\
\midrule
\endfirsthead
\caption[]{Counts of values of trained_on in final_deflattened_nonan_PRAUC} \\
\toprule
 trained\_on \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       1221 \\
        900 \\
        512 \\
        512 \\
        505 \\
        497 \\
        496 \\
        455 \\
        425 \\
        413 \\
        320 \\
        320 \\
        308 \\
        273 \\
        263 \\
        261 \\
        241 \\
        240 \\
        235 \\
        235 \\
        231 \\
        230 \\
        212 \\
        173 \\
        158 \\
        155 \\
        150 \\
        141 \\
        137 \\
        135 \\
        108 \\
         93 \\
         88 \\
         80 \\
         80 \\
         80 \\
         78 \\
         74 \\
         63 \\
         60 \\
         60 \\
         60 \\
         60 \\
         58 \\
         58 \\
         57 \\
         45 \\
         43 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         12 \\
         10 \\
         10 \\
          8 \\
          5 \\
          5 \\
          5 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_RCE-algorithm-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of algorithm in final_deflattened_nonan_RCE}
\label{tabfinal_deflattened_nonan_RCEalgorithm}\\
\toprule
 algorithm \\
\midrule
\endfirsthead
\caption[]{Counts of values of algorithm in final_deflattened_nonan_RCE} \\
\toprule
 algorithm \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
      4152 \\
      3771 \\
      2062 \\
      1707 \\
       174 \\
        73 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_RCE-eo_dataset-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of eo_dataset in final_deflattened_nonan_RCE}
\label{tabfinal_deflattened_nonan_RCEeo_dataset}\\
\toprule
 eo\_dataset \\
\midrule
\endfirsthead
\caption[]{Counts of values of eo_dataset in final_deflattened_nonan_RCE} \\
\toprule
 eo\_dataset \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       3870 \\
       3849 \\
       3804 \\
        416 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_RCE-eo_percent-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of eo_percent in final_deflattened_nonan_RCE}
\label{tabfinal_deflattened_nonan_RCEeo_percent}\\
\toprule
 eo\_percent \\
\midrule
\endfirsthead
\caption[]{Counts of values of eo_percent in final_deflattened_nonan_RCE} \\
\toprule
 eo\_percent \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       6583 \\
       2234 \\
       1591 \\
       1336 \\
        195 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_RCE-eo_technique-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of eo_technique in final_deflattened_nonan_RCE}
\label{tabfinal_deflattened_nonan_RCEeo_technique}\\
\toprule
 eo\_technique \\
\midrule
\endfirsthead
\caption[]{Counts of values of eo_technique in final_deflattened_nonan_RCE} \\
\toprule
 eo\_technique \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
         2752 \\
         2272 \\
         2264 \\
         2263 \\
         2193 \\
          195 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_RCE-evaluated_on-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of evaluated_on in final_deflattened_nonan_RCE}
\label{tabfinal_deflattened_nonan_RCEevaluated_on}\\
\toprule
 evaluated\_on \\
\midrule
\endfirsthead
\caption[]{Counts of values of evaluated_on in final_deflattened_nonan_RCE} \\
\toprule
 evaluated\_on \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
          479 \\
          473 \\
          455 \\
          427 \\
          425 \\
          425 \\
          424 \\
          424 \\
          424 \\
          420 \\
          418 \\
          417 \\
          417 \\
          413 \\
          413 \\
          213 \\
          213 \\
          213 \\
          127 \\
          127 \\
          127 \\
          127 \\
          127 \\
          126 \\
          123 \\
          123 \\
          123 \\
          123 \\
          118 \\
          118 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
          101 \\
           98 \\
           97 \\
           97 \\
           97 \\
           97 \\
           97 \\
           97 \\
           88 \\
           88 \\
           86 \\
           81 \\
           81 \\
           81 \\
           78 \\
           78 \\
           78 \\
           72 \\
           72 \\
           72 \\
           65 \\
           65 \\
           65 \\
           40 \\
           25 \\
           23 \\
           23 \\
           23 \\
           21 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           20 \\
           16 \\
           15 \\
           15 \\
           15 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_RCE-feature_selection-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of feature_selection in final_deflattened_nonan_RCE}
\label{tabfinal_deflattened_nonan_RCEfeature_selection}\\
\toprule
 feature\_selection \\
\midrule
\endfirsthead
\caption[]{Counts of values of feature_selection in final_deflattened_nonan_RCE} \\
\toprule
 feature\_selection \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
              4600 \\
              1987 \\
              1814 \\
              1802 \\
              1736 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_RCE-note-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of note in final_deflattened_nonan_RCE}
\label{tabfinal_deflattened_nonan_RCEnote}\\
\toprule
 note \\
\midrule
\endfirsthead
\caption[]{Counts of values of note in final_deflattened_nonan_RCE} \\
\toprule
 note \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
11308 \\
  631 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_RCE-to_dataset-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of to_dataset in final_deflattened_nonan_RCE}
\label{tabfinal_deflattened_nonan_RCEto_dataset}\\
\toprule
 to\_dataset \\
\midrule
\endfirsthead
\caption[]{Counts of values of to_dataset in final_deflattened_nonan_RCE} \\
\toprule
 to\_dataset \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       7661 \\
       2498 \\
       1058 \\
        722 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_RCE-to_percent-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of to_percent in final_deflattened_nonan_RCE}
\label{tabfinal_deflattened_nonan_RCEto_percent}\\
\toprule
 to\_percent \\
\midrule
\endfirsthead
\caption[]{Counts of values of to_percent in final_deflattened_nonan_RCE} \\
\toprule
 to\_percent \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       5128 \\
       4022 \\
       1606 \\
       1183 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_RCE-to_technique-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of to_technique in final_deflattened_nonan_RCE}
\label{tabfinal_deflattened_nonan_RCEto_technique}\\
\toprule
 to\_technique \\
\midrule
\endfirsthead
\caption[]{Counts of values of to_technique in final_deflattened_nonan_RCE} \\
\toprule
 to\_technique \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
         3885 \\
         2413 \\
         2353 \\
         2123 \\
         1165 \\
\end{longtable}


==> Tables/EvalValueCounts/final_deflattened_nonan_RCE-trained_on-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of trained_on in final_deflattened_nonan_RCE}
\label{tabfinal_deflattened_nonan_RCEtrained_on}\\
\toprule
 trained\_on \\
\midrule
\endfirsthead
\caption[]{Counts of values of trained_on in final_deflattened_nonan_RCE} \\
\toprule
 trained\_on \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       1221 \\
        900 \\
        512 \\
        512 \\
        505 \\
        497 \\
        496 \\
        455 \\
        425 \\
        413 \\
        320 \\
        320 \\
        308 \\
        273 \\
        263 \\
        261 \\
        241 \\
        240 \\
        235 \\
        235 \\
        231 \\
        230 \\
        212 \\
        173 \\
        158 \\
        155 \\
        150 \\
        141 \\
        137 \\
        135 \\
        108 \\
         93 \\
         88 \\
         80 \\
         80 \\
         80 \\
         78 \\
         74 \\
         63 \\
         60 \\
         60 \\
         60 \\
         60 \\
         58 \\
         58 \\
         57 \\
         45 \\
         43 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         15 \\
         12 \\
         10 \\
         10 \\
          8 \\
          5 \\
          5 \\
          5 \\
\end{longtable}


==> Tables/EvalValueCounts/final_flattened_RCE-eo_percent-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of eo_percent in final_flattened_RCE}
\label{tabfinal_flattened_RCEeo_percent}\\
\toprule
 eo\_percent \\
\midrule
\endfirsthead
\caption[]{Counts of values of eo_percent in final_flattened_RCE} \\
\toprule
 eo\_percent \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
      32910 \\
      11170 \\
       7955 \\
       6680 \\
        975 \\
\end{longtable}


==> Tables/EvalValueCounts/final_flattened_RCE-eo_technique-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of eo_technique in final_flattened_RCE}
\label{tabfinal_flattened_RCEeo_technique}\\
\toprule
 eo\_technique \\
\midrule
\endfirsthead
\caption[]{Counts of values of eo_technique in final_flattened_RCE} \\
\toprule
 eo\_technique \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
        13756 \\
        11360 \\
        11320 \\
        11315 \\
        10964 \\
          975 \\
\end{longtable}


==> Tables/EvalValueCounts/final_flattened_RCE-evaluated_on-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of evaluated_on in final_flattened_RCE}
\label{tabfinal_flattened_RCEevaluated_on}\\
\toprule
 evaluated\_on \\
\midrule
\endfirsthead
\caption[]{Counts of values of evaluated_on in final_flattened_RCE} \\
\toprule
 evaluated\_on \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
         2395 \\
         2361 \\
         2275 \\
         2135 \\
         2125 \\
         2125 \\
         2120 \\
         2120 \\
         2120 \\
         2100 \\
         2090 \\
         2085 \\
         2085 \\
         2065 \\
         2065 \\
         1065 \\
         1065 \\
         1065 \\
          635 \\
          635 \\
          635 \\
          635 \\
          635 \\
          630 \\
          615 \\
          615 \\
          615 \\
          615 \\
          590 \\
          590 \\
          505 \\
          505 \\
          505 \\
          505 \\
          505 \\
          505 \\
          505 \\
          505 \\
          505 \\
          505 \\
          505 \\
          490 \\
          485 \\
          485 \\
          485 \\
          485 \\
          485 \\
          485 \\
          440 \\
          440 \\
          430 \\
          405 \\
          405 \\
          405 \\
          390 \\
          390 \\
          390 \\
          360 \\
          360 \\
          360 \\
          325 \\
          325 \\
          325 \\
          200 \\
          125 \\
          115 \\
          115 \\
          115 \\
          104 \\
          100 \\
          100 \\
          100 \\
          100 \\
          100 \\
          100 \\
          100 \\
          100 \\
          100 \\
          100 \\
           80 \\
           75 \\
           75 \\
           75 \\
\end{longtable}


==> Tables/EvalValueCounts/final_flattened_RCE-feature_selection-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of feature_selection in final_flattened_RCE}
\label{tabfinal_flattened_RCEfeature_selection}\\
\toprule
 feature\_selection \\
\midrule
\endfirsthead
\caption[]{Counts of values of feature_selection in final_flattened_RCE} \\
\toprule
 feature\_selection \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
             22995 \\
              9935 \\
              9070 \\
              9010 \\
              8680 \\
\end{longtable}


==> Tables/EvalValueCounts/final_flattened_RCE-note-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of note in final_flattened_RCE}
\label{tabfinal_flattened_RCEnote}\\
\toprule
 note \\
\midrule
\endfirsthead
\caption[]{Counts of values of note in final_flattened_RCE} \\
\toprule
 note \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
56540 \\
 3150 \\
\end{longtable}


==> Tables/EvalValueCounts/final_flattened_RCE-to_dataset-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of to_dataset in final_flattened_RCE}
\label{tabfinal_flattened_RCEto_dataset}\\
\toprule
 to\_dataset \\
\midrule
\endfirsthead
\caption[]{Counts of values of to_dataset in final_flattened_RCE} \\
\toprule
 to\_dataset \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
      38304 \\
      12490 \\
       5286 \\
       3610 \\
\end{longtable}


==> Tables/EvalValueCounts/final_flattened_RCE-to_percent-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of to_percent in final_flattened_RCE}
\label{tabfinal_flattened_RCEto_percent}\\
\toprule
 to\_percent \\
\midrule
\endfirsthead
\caption[]{Counts of values of to_percent in final_flattened_RCE} \\
\toprule
 to\_percent \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
      25635 \\
      20110 \\
       8030 \\
       5915 \\
\end{longtable}


==> Tables/EvalValueCounts/final_flattened_RCE-to_technique-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of to_technique in final_flattened_RCE}
\label{tabfinal_flattened_RCEto_technique}\\
\toprule
 to\_technique \\
\midrule
\endfirsthead
\caption[]{Counts of values of to_technique in final_flattened_RCE} \\
\toprule
 to\_technique \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
        19424 \\
        12061 \\
        11765 \\
        10615 \\
         5825 \\
\end{longtable}


==> Tables/EvalValueCounts/final_flattened_RCE-trained_on-value_counts.tex <==
\begin{longtable}[ht]{r}
\caption{Counts of values of trained_on in final_flattened_RCE}
\label{tabfinal_flattened_RCEtrained_on}\\
\toprule
 trained\_on \\
\midrule
\endfirsthead
\caption[]{Counts of values of trained_on in final_flattened_RCE} \\
\toprule
 trained\_on \\
\midrule
\endhead
\midrule
\multicolumn{1}{r}{{Continued on next page}} \\
\midrule
\endfoot

\bottomrule
\endlastfoot
       6104 \\
       4500 \\
       2560 \\
       2560 \\
       2525 \\
       2485 \\
       2480 \\
       2275 \\
       2125 \\
       2065 \\
       1600 \\
       1600 \\
       1540 \\
       1365 \\
       1315 \\
       1305 \\
       1205 \\
       1200 \\
       1175 \\
       1175 \\
       1155 \\
       1150 \\
       1060 \\
        861 \\
        790 \\
        775 \\
        750 \\
        705 \\
        685 \\
        675 \\
        540 \\
        465 \\
        440 \\
        400 \\
        400 \\
        400 \\
        390 \\
        370 \\
        315 \\
        300 \\
        300 \\
        300 \\
        300 \\
        290 \\
        290 \\
        285 \\
        225 \\
        215 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         75 \\
         60 \\
         50 \\
         50 \\
         40 \\
         25 \\
         25 \\
         25 \\
\end{longtable}


==> Tables/Leaderboard/leaderboard+citatiotions.tex <==
\begin{tabular}{llllllllllll}
\toprule
Team/User Name &     Reference & Rank & Score & PRAUC Retweet & RCE Retweet & PRAUC Reply & RCE Reply & PRAUC Like & RCE Like & PRAUC comment & RCE comment \\
\midrule
NVIDIA RAPIDS.AI &  \cite{[CP7]} &    1 &     9 &        0.6111 &       37.91 &      0.2185 &     24.23 &     0.9108 &    53.01 &        0.0796 &        17.4 \\
learner          &  \cite{[CP9]} &    2 &    14 &        0.5395 &       30.96 &      0.2218 &     21.94 &     0.7761 &    25.42 &        0.0757 &       14.61 \\
Team Wantedly    &  \cite{[CP4]} &    3 &    18 &        0.5266 &       30.06 &      0.1918 &     20.44 &     0.7716 &    24.76 &        0.0724 &       14.86 \\
learner\_recsys   &  \cite{[CP3]} &    4 &    20 &        0.4529 &        22.5 &      0.1161 &     10.42 &     0.7221 &    18.28 &        0.5037 &       -0.04 \\
BanaNeverAlone   &  \cite{[CP6]} &    4 &    20 &        0.5042 &       27.21 &       0.185 &     18.71 &     0.7531 &     21.2 &        0.1237 &        8.34 \\
Los Trinadores   &  \cite{[CP8]} &    6 &    22 &        0.3673 &       16.93 &      0.5135 &     -0.04 &      0.731 &    20.09 &        0.5037 &          -0 \\
Not\_Last\_Place   &  \cite{[CP2]} &    9 &    28 &        0.4891 &        21.8 &      0.1761 &      18.6 &     0.7511 &    17.64 &        0.0516 &        10.3 \\
saaay71          &  \cite{[CP5]} &   28 &    63 &        0.1703 &        2.67 &      0.0593 &     -6.27 &     0.5879 &     7.21 &        0.0099 &      -62.98 \\
\bottomrule
\end{tabular}


\begin{table}[h]
    \centering
\begin{tabular}{lllll}
\toprule
Team/User Name & PRAUC Like & RCE Like & PRAUC Reply & RCE Reply \\
\midrule
NVIDIA RAPIDS.AI &     \textbf{0.9108} &    \textbf{53.01} &      0.2185 &     \textbf{24.23} \\
learner          &     0.7761 &    25.42 &      \textbf{0.2218} &     21.94 \\
Team Wantedly    &     0.7716 &    24.76 &      0.1918 &     20.44 \\
learner\_recsys   &     0.7221 &    18.28 &      0.1161 &     10.42 \\
BanaNeverAlone   &     0.7531 &     21.2 &       0.185 &     18.71 \\
Los Trinadores   &      0.731 &    20.09 &      0.5135 &     -0.04 \\
Not\_Last\_Place   &     0.7511 &    17.64 &      0.1761 &      18.6 \\
saaay71          &     0.5879 &     7.21 &      0.0593 &     -6.27 \\
\bottomrule
\end{tabular}
\caption{Scores for like and reply; notice the only case where \cite{[CP7]} did not achieve the best score}
\label{tabLeaderBoard2}
\end{table}



==> Tables/MostInformativeFeatures/Overview_of_the_25_and_50_most_informative_feature_as_selected_by_ChiSq-selector_on_the_train_dataset_and_its_20_subsets.tex <==
\begin{longtable}[ht]{lllr}
\caption{Overview of the 25 and 50 most informative feature as selected by ChiSq-selector on the train dataset and its 20 subsets} \label{tabOverview of the 25 and 50 most informative feature as selected by ChiSq-selector on the train dataset and its 20 subsets} \\
\toprule
 &  &  & count \\
target & features threshold & selected feature &  \\
\midrule
\endfirsthead
\caption[]{Overview of the 25 and 50 most informative feature as selected by ChiSq-selector on the train dataset and its 20 subsets} \\
\toprule
 &  &  & count \\
target & features threshold & selected feature &  \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
\hline \multirow[c]{27}{*}{like} & \hline \multirow[c]{27}{*}{top\_25} & language\_indexed & 21 \\
 &  & tweet\_type\_indexed & 21 \\
 &  & user\_domains\_frequency\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_negative\_tweets\_reply\_binned & 21 \\
 &  & user\_hashtags\_frequency\_1h\_binned & 21 \\
 &  & hashtags\_frequency\_1h\_binned & 21 \\
 &  & domains\_frequency\_48h\_binned & 21 \\
 &  & hashtags\_frequency\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_react\_binned & 21 \\
 &  & user\_links\_frequency\_2h\_binned & 21 \\
 &  & links\_frequency\_48h\_binned & 21 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_quote\_binned & 21 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_retweet\_binned & 21 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 21 \\
 &  & engageds\_tweets\_views\_count\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_reply\_binned & 21 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_retweet\_binned & 21 \\
 &  & user\_links\_frequency\_12h\_binned & 21 \\
 &  & engaging\_user\_follower\_count\_binned & 21 \\
 &  & user\_links\_frequency\_24h\_binned & 21 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_positive\_tweets\_react\_binned & 21 \\
 &  & ratio\_seen\_tweets\_in\_this\_langauge\_to\_total\_seen\_tweets\_binned & 21 \\
 &  & user\_hashtags\_frequency\_24h\_binned & 21 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 19 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 17 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_positive\_tweets\_quote\_binned & 5 \\
 &  & user\_domains\_frequency\_1h\_binned & 1 \\
\hline \multirow[c]{33}{*}{reply} & \hline \multirow[c]{33}{*}{top\_25} & language\_indexed & 21 \\
 &  & tweet\_type\_indexed & 21 \\
 &  & user\_domains\_frequency\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_negative\_tweets\_reply\_binned & 21 \\
 &  & user\_hashtags\_frequency\_1h\_binned & 21 \\
 &  & hashtags\_frequency\_1h\_binned & 21 \\
 &  & domains\_frequency\_48h\_binned & 21 \\
 &  & hashtags\_frequency\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_react\_binned & 21 \\
 &  & user\_links\_frequency\_2h\_binned & 21 \\
 &  & links\_frequency\_48h\_binned & 21 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_quote\_binned & 21 \\
 &  & engageds\_tweets\_views\_count\_12h\_binned & 21 \\
 &  & user\_links\_frequency\_12h\_binned & 21 \\
 &  & engaging\_user\_follower\_count\_binned & 21 \\
 &  & user\_links\_frequency\_24h\_binned & 21 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_positive\_tweets\_react\_binned & 21 \\
 &  & user\_hashtags\_frequency\_24h\_binned & 21 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 20 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 20 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_retweet\_binned & 20 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_reply\_binned & 19 \\
 &  & ratio\_seen\_tweets\_in\_this\_langauge\_to\_total\_seen\_tweets\_binned & 16 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_retweet\_binned & 15 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 14 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_positive\_tweets\_quote\_binned & 7 \\
 &  & user\_domains\_frequency\_1h\_binned & 6 \\
 &  & user\_domains\_frequency\_05h\_binned & 4 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_positive\_tweets\_retweet\_binned & 2 \\
 &  & engageds\_tweets\_views\_count\_24h\_binned & 1 \\
 &  & user\_links\_frequency\_48h\_binned & 1 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_positive\_tweets\_reply\_binned & 1 \\
 &  & user\_hashtags\_frequency\_05h\_binned & 1 \\
\hline \multirow[c]{29}{*}{retweet} & \hline \multirow[c]{29}{*}{top\_25} & language\_indexed & 21 \\
 &  & tweet\_type\_indexed & 21 \\
 &  & user\_domains\_frequency\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_negative\_tweets\_reply\_binned & 21 \\
 &  & user\_hashtags\_frequency\_1h\_binned & 21 \\
 &  & hashtags\_frequency\_1h\_binned & 21 \\
 &  & domains\_frequency\_48h\_binned & 21 \\
 &  & hashtags\_frequency\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_react\_binned & 21 \\
 &  & user\_links\_frequency\_2h\_binned & 21 \\
 &  & links\_frequency\_48h\_binned & 21 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_quote\_binned & 21 \\
 &  & engageds\_tweets\_views\_count\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 21 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_reply\_binned & 21 \\
 &  & user\_links\_frequency\_12h\_binned & 21 \\
 &  & engaging\_user\_follower\_count\_binned & 21 \\
 &  & user\_links\_frequency\_24h\_binned & 21 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_positive\_tweets\_react\_binned & 21 \\
 &  & ratio\_seen\_tweets\_in\_this\_langauge\_to\_total\_seen\_tweets\_binned & 21 \\
 &  & user\_hashtags\_frequency\_24h\_binned & 21 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_retweet\_binned & 20 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 20 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_retweet\_binned & 20 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 17 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_positive\_tweets\_quote\_binned & 4 \\
 &  & user\_domains\_frequency\_1h\_binned & 1 \\
 &  & user\_domains\_frequency\_05h\_binned & 1 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_positive\_tweets\_retweet\_binned & 1 \\
\hline \multirow[c]{84}{*}{quote} & \hline \multirow[c]{84}{*}{top\_25} & language\_indexed & 21 \\
 &  & engaging\_user\_follower\_count\_binned & 21 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_positive\_tweets\_react\_binned & 19 \\
 &  & tweet\_type\_indexed & 19 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_retweet\_binned & 18 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_react\_binned & 17 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_quote\_binned & 16 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 16 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_negative\_tweets\_reply\_binned & 16 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_positive\_tweets\_quote\_binned & 15 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 15 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_retweet\_binned & 15 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 14 \\
 &  & hashtags\_frequency\_12h\_binned & 14 \\
 &  & engageds\_tweets\_views\_count\_12h\_binned & 14 \\
 &  & user\_hashtags\_frequency\_1h\_binned & 14 \\
 &  & user\_hashtags\_frequency\_24h\_binned & 14 \\
 &  & hashtags\_frequency\_1h\_binned & 13 \\
 &  & links\_frequency\_48h\_binned & 13 \\
 &  & domains\_frequency\_48h\_binned & 12 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_positive\_tweets\_retweet\_binned & 11 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_reply\_binned & 10 \\
 &  & user\_domains\_frequency\_12h\_binned & 10 \\
 &  & user\_links\_frequency\_2h\_binned & 10 \\
 &  & user\_links\_frequency\_12h\_binned & 10 \\
 &  & user\_links\_frequency\_24h\_binned & 10 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_positive\_tweets\_retweet\_binned & 8 \\
 &  & engageds\_tweets\_views\_count\_24h\_binned & 8 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_positive\_tweets\_react\_binned & 7 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_positive\_tweets\_reply\_binned & 7 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_like\_binned & 5 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_like\_binned & 5 \\
 &  & user\_hashtags\_frequency\_05h\_binned & 5 \\
 &  & user\_hashtags\_frequency\_2h\_binned & 5 \\
 &  & ratio\_all\_to\_engaging\_count\_negative\_tweets\_quote\_binned & 5 \\
 &  & ratio\_all\_to\_engaging\_count\_negative\_tweets\_retweet\_binned & 5 \\
 &  & engageds\_tweets\_views\_count\_48h\_binned & 4 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_reply\_binned & 4 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_negative\_tweets\_retweet\_binned & 4 \\
 &  & engaging\_user\_following\_count\_binned & 4 \\
 &  & ratio\_engaged\_to\_engaging\_follower\_counts\_binned & 4 \\
 &  & engaged\_with\_user\_follower\_count\_binned & 4 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_react\_binned & 3 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_reply\_binned & 3 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_negative\_tweets\_quote\_binned & 3 \\
 &  & engagee\_follows\_engager & 3 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_negative\_tweets\_react\_binned & 2 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_positive\_tweets\_retweet\_binned & 2 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_positive\_tweets\_like\_binned & 2 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_positive\_tweets\_react\_binned & 2 \\
 &  & ratio\_engaged\_to\_engaging\_following\_counts\_binned & 2 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_like\_binned & 2 \\
 &  & ratio\_all\_to\_engaging\_count\_negative\_tweets\_like\_binned & 2 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_positive\_tweets\_quote\_binned & 2 \\
 &  & domains\_frequency\_24h\_binned & 2 \\
 &  & user\_domains\_frequency\_1h\_binned & 2 \\
 &  & engageds\_tweets\_views\_count\_05h\_binned & 2 \\
 &  & engageds\_tweets\_views\_count\_2h\_binned & 2 \\
 &  & engageds\_tweets\_views\_count\_1h\_binned & 2 \\
 &  & engaging\_user\_is\_verified & 2 \\
 &  & engaged\_with\_user\_is\_verified & 1 \\
 &  & graph\_engaged\_flag\_quote\_from\_engaging\_1d & 1 \\
 &  & graph\_engaged\_count\_quote\_from\_engaging\_1d & 1 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_positive\_tweets\_like\_binned & 1 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_react\_binned & 1 \\
 &  & domains\_frequency\_2h\_binned & 1 \\
 &  & ratio\_all\_to\_engaging\_count\_negative\_tweets\_reply\_binned & 1 \\
 &  & ratio\_all\_to\_engaging\_count\_negative\_tweets\_react\_binned & 1 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_quote\_binned & 1 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_negative\_tweets\_react\_binned & 1 \\
 &  & hashtags\_frequency\_05h\_binned & 1 \\
 &  & hashtags\_frequency\_24h\_binned & 1 \\
 &  & hashtags\_frequency\_48h\_binned & 1 \\
 &  & hashtags\_frequency\_2h\_binned & 1 \\
 &  & links\_frequency\_24h\_binned & 1 \\
 &  & user\_domains\_frequency\_05h\_binned & 1 \\
 &  & user\_links\_frequency\_48h\_binned & 1 \\
 &  & user\_domains\_frequency\_48h\_binned & 1 \\
 &  & user\_links\_frequency\_1h\_binned & 1 \\
 &  & graph\_engaged\_count\_like\_from\_engaging\_2d & 1 \\
 &  & graph\_engaged\_count\_react\_from\_engaging\_2d & 1 \\
 &  & graph\_engagee\_follows\_engager\_2d & 1 \\
 &  & engaged\_with\_user\_following\_count\_binned & 1 \\
 &  & ratio\_seen\_tweets\_in\_this\_langauge\_to\_total\_seen\_tweets\_binned & 1 \\
\hline \multirow[c]{27}{*}{react} & \hline \multirow[c]{27}{*}{top\_25} & language\_indexed & 21 \\
 &  & tweet\_type\_indexed & 21 \\
 &  & user\_domains\_frequency\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_negative\_tweets\_reply\_binned & 21 \\
 &  & user\_hashtags\_frequency\_1h\_binned & 21 \\
 &  & hashtags\_frequency\_1h\_binned & 21 \\
 &  & domains\_frequency\_48h\_binned & 21 \\
 &  & hashtags\_frequency\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_react\_binned & 21 \\
 &  & user\_links\_frequency\_2h\_binned & 21 \\
 &  & links\_frequency\_48h\_binned & 21 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_quote\_binned & 21 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_retweet\_binned & 21 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 21 \\
 &  & engageds\_tweets\_views\_count\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_reply\_binned & 21 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_retweet\_binned & 21 \\
 &  & user\_links\_frequency\_12h\_binned & 21 \\
 &  & engaging\_user\_follower\_count\_binned & 21 \\
 &  & user\_links\_frequency\_24h\_binned & 21 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_positive\_tweets\_react\_binned & 21 \\
 &  & ratio\_seen\_tweets\_in\_this\_langauge\_to\_total\_seen\_tweets\_binned & 21 \\
 &  & user\_hashtags\_frequency\_24h\_binned & 21 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 19 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 17 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_positive\_tweets\_quote\_binned & 5 \\
 &  & user\_domains\_frequency\_1h\_binned & 1 \\
\end{longtable}


==> Tables/MostInformativeFeatures/Overview_of_the_5_and_10_most_informative_feature_as_selected_by_ChiSq-selector_on_the_train_dataset_and_its_20_subsets.tex <==
\begin{longtable}[ht]{lllr}
\caption{Overview of the 5 and 10 most informative feature as selected by ChiSq-selector on the train dataset and its 20 subsets} \label{tabOverview of the 5 and 10 most informative feature as selected by ChiSq-selector on the train dataset and its 20 subsets} \\
\toprule
 &  &  & count \\
target & features threshold & selected feature &  \\
\midrule
\endfirsthead
\caption[]{Overview of the 5 and 10 most informative feature as selected by ChiSq-selector on the train dataset and its 20 subsets} \\
\toprule
 &  &  & count \\
target & features threshold & selected feature &  \\
\midrule
\endhead
\midrule
\multicolumn{4}{r}{Continued on next page} \\
\midrule
\endfoot
\bottomrule
\endlastfoot
\hline \multirow[c]{6}{*}{like} & \hline \multirow[c]{6}{*}{top\_5} & language\_indexed & 21 \\
 &  & tweet\_type\_indexed & 21 \\
 &  & user\_domains\_frequency\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_negative\_tweets\_reply\_binned & 21 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 17 \\
 &  & user\_hashtags\_frequency\_1h\_binned & 4 \\
\hline \multirow[c]{6}{*}{reply} & \hline \multirow[c]{6}{*}{top\_5} & language\_indexed & 21 \\
 &  & tweet\_type\_indexed & 21 \\
 &  & user\_domains\_frequency\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_negative\_tweets\_reply\_binned & 21 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 14 \\
 &  & user\_hashtags\_frequency\_1h\_binned & 7 \\
\hline \multirow[c]{6}{*}{retweet} & \hline \multirow[c]{6}{*}{top\_5} & language\_indexed & 21 \\
 &  & tweet\_type\_indexed & 21 \\
 &  & user\_domains\_frequency\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_negative\_tweets\_reply\_binned & 21 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 17 \\
 &  & user\_hashtags\_frequency\_1h\_binned & 4 \\
\hline \multirow[c]{18}{*}{quote} & \hline \multirow[c]{18}{*}{top\_5} & language\_indexed & 21 \\
 &  & tweet\_type\_indexed & 18 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 15 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_negative\_tweets\_reply\_binned & 15 \\
 &  & user\_domains\_frequency\_12h\_binned & 10 \\
 &  & user\_hashtags\_frequency\_1h\_binned & 5 \\
 &  & engaging\_user\_follower\_count\_binned & 4 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_react\_binned & 3 \\
 &  & ratio\_all\_to\_hashtags\_user\_proxy\_count\_positive\_tweets\_quote\_binned & 3 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_retweet\_binned & 2 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_positive\_tweets\_retweet\_binned & 2 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_positive\_tweets\_react\_binned & 1 \\
 &  & domains\_frequency\_24h\_binned & 1 \\
 &  & ratio\_all\_to\_engaging\_count\_positive\_tweets\_reply\_binned & 1 \\
 &  & ratio\_all\_to\_domains\_user\_proxy\_count\_negative\_tweets\_retweet\_binned & 1 \\
 &  & engageds\_tweets\_views\_count\_12h\_binned & 1 \\
 &  & domains\_frequency\_48h\_binned & 1 \\
 &  & ratio\_all\_to\_engaging\_count\_negative\_tweets\_quote\_binned & 1 \\
\hline \multirow[c]{6}{*}{react} & \hline \multirow[c]{6}{*}{top\_5} & language\_indexed & 21 \\
 &  & tweet\_type\_indexed & 21 \\
 &  & user\_domains\_frequency\_12h\_binned & 21 \\
 &  & ratio\_all\_to\_engaged\_with\_count\_negative\_tweets\_reply\_binned & 21 \\
 &  & ratio\_all\_to\_links\_user\_proxy\_count\_negative\_tweets\_quote\_binned & 17 \\
 &  & user\_hashtags\_frequency\_1h\_binned & 4 \\
\end{longtable}


==> Tables/datasetTables.tex <==
\begin{longtable}{|l|l|l|l|}
\caption{Number of instances and unique tweets as well as the ratios between the two for each dataset}
\label{tabDataset1}\\ 
\hline
\textbf{Dataset} & \textbf{no. of instances} & \textbf{no. of tweets} & \textbf{\#inst./\#tw.}  \endfirsthead 
\hline
\textbf{train}   & $141\ 748\ 660$         & $69\ 680\ 733$       & $2.03$                \\ 
\hline
\textbf{val}     & $10\ 271\ 157$          & $7\ 042\ 109$        & $1.46$                \\ 
\hline
\textbf{test}    & $10\ 350\ 033$          & $7\ 096\ 161$        & $1.46$                \\
\hline
\end{longtable}

\begin{longtable}{|l|l|l|l|l|}
\caption{Number of unique authors and viewers (engaged-with and engaging uswers) and the ratio of these to the total number of instances in each dataset}
\label{tabDataset2}\\ 
\hline
\textbf{Dataset} & \textbf{no. of authors} & \textbf{\#inst./\#auth.} & \textbf{no. of viewers} & \textbf{\#inst./\#vie.}  \endfirsthead 
\hline
\textbf{train}   & $14\ 471\ 617$        & $9.79$                 & $24\ 929\ 665$        & $5.69$                 \\ 
\hline
\textbf{val}     & $2\ 772\ 099$         & $3.71$                 & $5\ 597\ 372$         & $1.83$                 \\ 
\hline
\textbf{test}             & $2\ 794\ 081$         & $3.70$                 & $5\ 633\ 471$         & $1.84$                 \\
\hline
\end{longtable}

==> appx3.tex <==
\chapter{Source Code Snippets}
\label{appSourceCodeSnippets}

This appendix contains code snippets that might be of interest for reproducibility or extension attempts.

\section{Snippets from Feature Engineering}
\label{appSnippetsFromFeatureEngineering}

Listing in \ref{lstDecodeText} de-tokenises tweet text and was originally used in the notebook \texttt{PySpark\--Feature\-Eng\--00\--Feature\-Eng}.

\input{Listings/ForAppendix/decodingText}

The listings in \ref{lst1dFollows} and \ref{lst2dFollows} showcase how the first degree and second degree graphs (in tabular representation were created). Listing in \ref{lstExtractNewRelations} shows how the graph relations were then finally joined back with the main dataframe.

\input{Listings/ForAppendix/1dFollows}

\input{Listings/ForAppendix/2dFollows}

\input{Listings/ForAppendix/extractGraphRelations}

The main idea for features in \texttt{03-TimeFeatures} was to investigate trends in the last past 30 minutes, 60 minutes, and 120 minutes, as well as 12 hours, 24 hours, and 48 hours before the tweet was seen. Since val, and test datasets contain tweets from the week following the week in the train dataset, the first step was to append the last two days from train to val, test, val+test and all their subsets, which was done in the method in listing \ref{lstLast48h}.

\input{Listings/ForAppendix/last48h}

Implementing feature in \texttt{03-TimeFeatures} was challenging as the Window function did not have all of its functionalities available in the dataframe API version of PySpark. Listing \ref{lstGetFrequency} below contains the function that counted recent tweet elements and is illustrative of the overall approach together taken. In its comments it also contain links that showcase what the result of each step is. The helper-function \texttt{re\-solve\-'\_col\-umn\-\_naming} is omitted from the report here, as it only perform a simple and task-specific column name checking and manipulation.

\input{Listings/ForAppendix/getFrequency}

As was elaborated in subsection \ref{secTweetElementsEngagementHistory}, there are no tweets that appear in both the train dataset as well as the val and test datasets, which is why we used the \texttt{engaged\-\_with\-\_user\-\_id} instead of the \texttt{tweet\-\_id}. The function that was used to achieve this can be seen in listing \ref{lstUserProxy}.

\input{Listings/ForAppendix/userProxy}

\section{Snippets from Feature Selection}
\label{appSnippetsFromFeatureSelection}

The part of the source code where the \texttt{Chi\-Sq\-Select\-or} is applied on all combinations of explanatory features and target engagements can be seen in listing \ref{lstChiSqSelecor}. 

\input{Listings/ForAppendix/chiSqSelector}

The method \texttt{fs\-vector\-ise\-\_select\-ed\-\_columns}, which can be seen in listing \ref{lstVectorisation}, selects the most informative columns. The results must then be turned in vectorised columns. Vectorised columns are columns with \texttt{Vector} data type, an array or list-like Spark data type. \texttt{Vector} is the required input format for MLLib classifiers (cf. \cite{mlbMLWithPyspark2019chapter3dataProcessing}). 

\input{Listings/ForAppendix/vectoriseSelectedColumns}

\section{Snippets from Classification and Evaluation}
\label{appSnippetsFromClassification and Evaluation}

The method in listing \ref{lstPredictEvaluate} tunes hyperparametres and fits initial models as well as generates initial predictions and evaluations. 

\input{Listings/ForAppendix/predictAndEvaluate}

The method in listing \ref{lstEvaluateAll} is the main part of program \texttt{Py\-Spark\-Pre\-dictions\--01\--In\-i\-tial\-Classification} and module \texttt{pp\-\_ml\-lib\-\_evaluate\-\_all}. The method creates and evaluates further predictions, as is elaborated in subsections \ref{secEvaluation} and \ref{secClassification}.

\input{Listings/ForAppendix/evaluateAll}

The method in listing \ref{lstGetCommonFactorCombinations} finds the common combinations of other factors for each value in the target factor, as explained in more detail in subsection \ref{secStatist}

\input{Listings/ForAppendix/getCommonFactorCombinations}

==> latexIntro.tex <==
%% intro.tex
%% Copyright (C) 2014-2020 by Thomas Auzinger <thomas@auzinger.name>
%
% This work may be distributed and/or modified under the
% conditions of the LaTeX Project Public License, either version 1.3
% of this license or (at your option) any later version.
% The latest version of this license is in
%   http://www.latex-project.org/lppl.txt
% and version 1.3 or later is part of all distributions of LaTeX
% version 2005/12/01 or later.
%
% This work has the LPPL maintenance status `maintained'.
%
% The Current Maintainer of this work is Thomas Auzinger.
%
% This work consists of the files vutinfth.dtx and vutinfth.ins
% and the derived file vutinfth.cls.
% This work also consists of the file intro.tex.


\newacronym{ctan}{CTAN}{Comprehensive TeX Archive Network}
\newacronym{faq}{FAQ}{Frequently Asked Questions}
\newacronym{pdf}{PDF}{Portable Document Format}
\newacronym{svn}{SVN}{Subversion}
\newacronym{wysiwyg}{WYSIWYG}{What You See Is What You Get}

\newglossaryentry{texteditor}
{
  name={editor},
  description={A text editor is a type of program used for editing plain text files.}
}

\chapter{Introduction to \LaTeX}

Since \LaTeX\ is widely used in academia and industry, there exists a plethora of freely accessible introductions to the language.
Reading through the guide at \url{https://en.wikibooks.org/wiki/LaTeX} serves as a comprehensive overview for most of the functionality and is highly recommended before starting with a thesis in \LaTeX.

\section{Installation}

A full \LaTeX\ distribution\index{distribution} consists not only of the binaries that convert the source files to the typeset documents, but also of a wide range of packages and their documentation.
Depending on the operating system, different implementations are available as shown in Table~\ref{tab:distrib}.
\textbf{Due to the large amount of packages that are in everyday use and due to their high interdependence, it is paramount to keep the installed distribution\index{distribution} up to date.}
Otherwise, obscure errors and tedious debugging ensue.

\begin{table}
  \centering
  \begin{tabular}{cccc}
    \toprule
    Distribution & Unix         & Windows      & MacOS        \\
    \midrule
    TeX Live     & \textbf{yes} & yes          & (yes)        \\
    MacTeX       & no           & no           & \textbf{yes} \\
    MikTeX       & (yes)        & \textbf{yes} & yes          \\
    \bottomrule
  \end{tabular}
  \caption{\TeX/\LaTeX\ distributions for different operating systems. Recomended choice in \textbf{bold}.}
  \label{tab:distrib} % \label has to be placed AFTER \caption to produce correct cross-references.
\end{table}

\section{Editors}

A multitude of \TeX\ \glspl{texteditor} are available differing in their editing models, their supported operating systems and their feature sets.
A comprehensive overview of \glspl{texteditor} can be found at the Wikipedia page  \url{https://en.wikipedia.org/wiki/Comparison_of_TeX_editors}.
TeXstudio (\url{http://texstudio.sourceforge.net/}) is recommended.
Most editors support a synchronization of the generated document and the \LaTeX\ source by \verb|Ctrl| clicking either on the source document or the generated document.

\section{Compilation}

Modern editors usually provide the compilation programs to generate \gls{pdf} documents and for most \LaTeX\ source files, this is sufficient.
More advanced \LaTeX\ functionality, such as glossaries and bibliographies, needs additional compilation steps, however.
It is also possible that errors in the compilation process invalidate intermediate files and force subsequent compilation runs to fail.
It is advisable to delete intermediate files (\verb|.aux|, \verb|.bbl|, etc.), if errors occur and persist.
All files that are not generated by the user are automatically regenerated.
To compile the current document, the steps as shown in Table~\ref{tab:compile} have to be taken.


\begin{table}
  \centering
  \begin{tabular}{rl}
    \toprule
    & Description \\
    \midrule
    1 & Scan for refs, toc/lof/lot/loa items and cites \\
    2 & Build the bibliography     \\
    3 & Link refs and build the toc/lof/lot/loa \\
    4 & Link the bibliography \\
    5 & Build the glossary \\
    6 & Build the acronyms \\
    7 & Build the index \\
    8 & Link the glossary, acronyms, and the index \\
    9 & Link the bookmarks \\
    \midrule
    & Command \\
    \midrule
    1 & \verb|pdflatex.exe  example| \\
    2 & \verb|bibtex.exe    example| \\
    3 & \verb|pdflatex.exe  example| \\
    4 & \verb|pdflatex.exe  example| \\
    5 & \verb|makeindex.exe -t example.glg -s example.ist| \\
      & \verb|              -o example.gls example.glo| \\
    6 & \verb|makeindex.exe -t example.alg -s example.ist| \\
      & \verb|              -o example.acr example.acn| \\
    7 & \verb|makeindex.exe -t example.ilg -o example.ind example.idx| \\
    8 & \verb|pdflatex.exe  example| \\
    9 & \verb|pdflatex.exe  example| \\
    \bottomrule
  \end{tabular}
  \caption{Compilation steps for this document. The following abbreviations were used: table of contents (toc), list of figures (lof), list of tables (lot), list of algorithms (loa).}
  \label{tab:compile} % \label has to be placed AFTER \caption to produce correct cross-references.
\end{table}


\section{Basic Functionality}

In this section, various examples are given of the fundamental building blocks used in a thesis.
Many \LaTeX\ commands have a rich set of options that can be supplied as optional arguments.
The documentation of each command should be consulted to get an impression of the full spectrum of its functionality.

\subsection{Floats}

Two main categories of page elements can be differentiated in the usual \LaTeX\ workflow: \textit{(i)} the main stream of text and \textit{(ii)} floating containers that are positioned at convenient positions throughout the document.
In most cases, tables, plots, and images are put into such containers since they are usually positioned at the top or bottom of pages.
These are realized by the two environments \verb|figure| and \verb|table|, which also provide functionality for cross-referencing (see Table~\ref{tab:intro} and Figure~\ref{fig:intro}) and the generation of corresponding entries in the list of figures and the list of tables.
Note that these environments solely act as containers and can be assigned arbitrary content.

\subsection{Tables}

A table in \LaTeX\ is created by using a \verb|tabular| environment or any of its extensions, e.g., \verb|tabularx|.
The commands \verb|\multirow| and \verb|\multicolumn| allow table elements to span multiple rows and columns.

\begin{table}[h] % placement specifier
  \centering
  \begin{tabular}{lll}
    \toprule
    \multicolumn{2}{c}{Position} \\
    \cmidrule{1-2} % partial horizontal rule
    Group & Abbrev & Name \\
    \midrule
    Goalkeeper & GK & Paul Robinson \\
    \midrule
    \multirow{4}{*}{Defenders} & LB & Lucus Radebe \\
                               & DC & Michael Duburry \\
                               & DC & Dominic Matteo \\
                               & RB & Didier Domi \\
    \midrule
    \multirow{3}{*}{Midfielders} & MC & David Batty \\
                                 & MC & Eirik Bakke \\
                                 & MC & Jody Morris \\
    \midrule
    Forward & FW & Jamie McMaster \\
    \midrule
    \multirow{2}{*}{Strikers} & ST & Alan Smith \\
                              & ST & Mark Viduka \\
    \bottomrule
  \end{tabular}
  \caption{Adapted example from the \LaTeX guide at \url{https://en.wikibooks.org/wiki/LaTeX/Tables}. This example uses rules specific to the \texttt{booktabs} package and employs the multi-row functionality of the \texttt{multirow} package.}
  \label{tab:intro} % \label has to be placed AFTER \caption to produce correct cross-references.
\end{table}

\subsection{Images}

An image is added to a document via the \verb|\includegraphics| command as shown in Figure~\ref{fig:intro}.
The \verb|\subcaption| command can be used to reference subfigures, such as Figure~\ref{fig:intro:full width} and~\ref{fig:intro:half width}.

\begin{figure}[h]
  \centering
  \begin{subfigure}[b]{0.45\columnwidth}
    \centering
    \includegraphics[width=\textwidth]{Logo-schwarz.pdf}
    \subcaption{The header logo at text width.}
    \label{fig:intro:full width}
  \end{subfigure}
  \begin{subfigure}[b]{0.45\columnwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{Logo-schwarz.pdf}
    \subcaption{The header logo at half the text width.}
    \label{fig:intro:half width}
  \end{subfigure}
  \caption[Optional caption for the figure list (often used to abbreviate long captions)]{The header logo at different sizes.} % Remove the [...] argument if the original caption should be used in the figure list.
  \label{fig:intro} % \label has to be placed AFTER \caption (or \subcaption) to produce correct cross-references.
\end{figure}

\subsection{Mathematical Expressions}

One of the original motivation to create the \TeX\ system was the need for mathematical typesetting.
To this day, \LaTeX\ is the preferred system to write math-heavy documents and a wide variety of functions aids the author in this task.
A mathematical expression can be inserted inline as $\sum_{n=1}^{\infty} \frac{1}{n^2} = \frac{\pi^2}{6}$ outside of the text stream as \[ \sum_{n=1}^{\infty} \frac{1}{n^2} = \frac{\pi^2}{6} \] or as numbered equation with
\begin{equation}
\sum_{n=1}^{\infty} \frac{1}{n^2} = \frac{\pi^2}{6}.
\end{equation}

\subsection{Pseudo Code}

The presentation of algorithms can be achieved with various packages; the most popular are \verb|algorithmic|, \verb|algorithm2e|, \verb|algorithmicx|, or \verb|algpseudocode|.
An overview is given at \url{https://tex.stackexchange.com/questions/229355}.
An example of the use of the \verb|alogrithm2e| package is given with Algorithm~\ref{alg:gauss-seidel}.

\begin{algorithm}
  \SetKw{BreakFor}{break for}
  \KwIn{A scalar~$\epsilon$, a matrix $\mathbf{A} = (a_{ij})$, a vector $\vec{b}$, and an initial vector $\vec{x}^{(0)}$}
  \KwOut{$\vec{x}^{(n)}$ with $\mathbf{A} \vec{x}^{(n)} \approx \vec{b}$}
  \For{$k\leftarrow 1$ \KwTo maximum iterations}
  {
     \For{$i\leftarrow 1$ \KwTo $n$}
     {
        $x_i^{(k)} = \frac{1}{a_{ii}} \left(b_i-\sum_{j<i} a_{ij} x_j^{(k)} - \sum_{j>i} a_{ij} x_j^{(k-1)} \right)$\;
     }
     \If{$\lvert\vec{x}^{(k)}-\vec{x}^{(k-1)}\rvert < \epsilon$}
     {\BreakFor\;}
  }
  \Return{$\vec{x}^{(k)}$\;}
  \caption{Gauss-Seidel}
  \label{alg:gauss-seidel} % \label has to be placed AFTER \caption to produce correct cross-references.
\end{algorithm}

\section{Bibliography}

The referencing of prior work is a fundamental requirement of academic writing and well supported by \LaTeX.
The \textsc{Bib}\TeX\ reference management software is the most commonly used system for this purpose.
Using the \verb|\cite| command, it is possible to reference entries in a \verb|.bib| file out of the text stream, e.g., as~\cite{Turing1936}.
The generation of the formatted bibliography needs a separate execution of \verb|bibtex.exe| (see Table~\ref{tab:compile}).

\section{Table of Contents}

The table of contents is automatically built by successive runs of the compilation, e.g., of \verb|pdflatex.exe|.
The command \verb|\setsecnumdepth| allows the specification of the depth of the table of contents and additional entries can be added to the table of contents using \verb|\addcontentsline|.
The starred versions of the sectioning commands, i.e., \verb|\chapter*|, \verb|\section*|, etc., remove the corresponding entry from the table of contents.

\section{Acronyms / Glossary / Index}

The list of acronyms, the glossary, and the index need to be built with a separate execution of \verb|makeindex| (see Table~\ref{tab:compile}).
Acronyms have to be specified with \verb|\newacronym| while glossary entries use \verb|\newglossaryentry|.
Both are then used in the document content with one of the variants of \verb|\gls|, such as \verb|\Gls|, \verb|\glspl|, or \verb|\Glspl|.
Index items are simply generated by placing \verb|\index|\marg{entry} next to all the words that correspond to the index entry \meta{entry}.
Note that many enhancements exist for these functionalities and the documentation of the \verb|makeindex| and the \verb|glossaries| packages should be consulted.

\section{Tips}

Since \TeX\ and its successors do not employ a \gls{wysiwyg} editing scheme, several guidelines improve the readability of the source content:
\begin{itemize}
\item Each sentence in the source text should start with a new line.
      This helps not only the user navigation through the text, but also enables revision control systems (e.g. \gls{svn}, Git) to show the exact changes authored by different users.
      Paragraphs are separated by one (or more) empty lines.
\item Environments, which are defined by a matching pair of \verb|\begin{name}| and \verb|\end{name}|, can be indented by whitespace to show their hierarchical structure.
\item In most cases, the explicit use of whitespace (e.g. by adding \verb|\hspace{4em}| or \verb|\vspace{1.5cm}|) violates typographic guidelines and rules.
      Explicit formatting should only be employed as a last resort and, most likely, better ways to achieve the desired layout can be found by a quick web search.
\item The use of bold or italic text is generally not supported by typographic considerations and the semantically meaningful \verb|\emph{|\texttt{$\dots$}\verb|}| should be used.
\end{itemize}

The predominant application of the \LaTeX\ system is the generation of \gls{pdf} files via the \textsc{Pdf}\LaTeX\ binaries.
In the current version of \textsc{Pdf}\LaTeX, it is possible that absolute file paths and user account names are embedded in the final \gls{pdf} document.
While this poses only a minor security issue for all documents, it is highly problematic for double blind reviews.
The process shown in Table~\ref{tab:ps2pdf} can be employed to strip all private information from the final \gls{pdf} document.

\begin{table}[h]
  \centering
  \begin{tabular}{rl}
  \toprule
  & Command \\
  \midrule
  1 & Rename the \gls{pdf} document \verb|final.pdf| to \verb|final.ps|. \\
  2 & Execute the following command: \\
    & \verb|ps2pdf -dPDFSETTINGS#/prepress ^| \\
    & \verb| -dCompatibilityLevel#1.4 ^| \\
    & \verb| -dAutoFilterColorImages#false ^| \\
    & \verb| -dAutoFilterGrayImages#false ^| \\
    & \verb| -dColorImageFilter#/FlateEncode ^| \\
    & \verb| -dGrayImageFilter#/FlateEncode ^| \\
    & \verb| -dMonoImageFilter#/FlateEncode ^| \\
    & \verb| -dDownsampleColorImages#false ^| \\
    & \verb| -dDownsampleGrayImages#false ^| \\
    & \verb| final.ps final.pdf| \\
  \bottomrule
  \end{tabular}

  On Unix-based systems, replace \verb|#| with \verb|=| and \verb|^| with \verb|\|.
  \caption{Anonymization of \gls{pdf} documents.}
  \label{tab:ps2pdf}
\end{table}

\section{Resources}

\subsection{Useful Links}

In the following, a listing of useful web resources is given.
\begin{description}
\item[\url{https://en.wikibooks.org/wiki/LaTeX}] An extensive wiki-based guide to \LaTeX.
\item[\url{http://www.tex.ac.uk/faq}] A (huge) set of \gls{faq} about \TeX\ and \LaTeX.
\item[\url{https://tex.stackexchange.com/}] The definitive user forum for non-trivial \LaTeX-related questions and answers.
\end{description}

\subsection[Comprehensive TeX Archive Network]{\gls{ctan}}

The \gls{ctan} is the official repository for all \TeX\ related material.
It can be accessed via \url{https://www.ctan.org/} and hosts (among other things) a huge variety of packages that provide extended functionality for \TeX\ and its successors.
Note that most packages contain \gls{pdf} documentation that can be directly accessed via \gls{ctan}.

In the following, a short, non-exhaustive list of relevant \gls{ctan}-hosted packages is given together with their relative path.
\begin{description}[itemsep=0ex]
\item[\href{https://www.ctan.org/pkg/algorithm2e}{algorithm2e}] Functionality for writing pseudo code.
\item[\href{https://www.ctan.org/pkg/amsmath}{amsmath}] Enhanced functionality for typesetting mathematical expressions.
\item[\href{https://www.ctan.org/pkg/amsfonts}{amssymb}] Provides a multitude of mathematical symbols.
\item[\href{https://www.ctan.org/pkg/booktabs}{booktabs}] Improved typesetting of tables.
\item[\href{https://www.ctan.org/pkg/enumitem}{enumitem}] Control over the layout of lists (\verb|itemize|, \verb|enumerate|, \verb|description|).
\item[\href{https://www.ctan.org/pkg/fontenc}{fontenc}] Determines font encoding of the output.
\item[\href{https://www.ctan.org/pkg/glossaries}{glossaries}] Create glossaries and list of acronyms.
\item[\href{https://www.ctan.org/pkg/graphicx}{graphicx}] Insert images into the document.
\item[\href{https://www.ctan.org/pkg/inputenc}{inputenc}] Determines encoding of the input.
\item[\href{https://www.ctan.org/pkg/l2tabu}{l2tabu}] A description of bad practices when using \LaTeX.
\item[\href{https://www.ctan.org/pkg/mathtools}{mathtools}] Further extension of mathematical typesetting.
\item[\href{https://www.ctan.org/pkg/memoir}{memoir}] The document class on upon which the \verb|vutinfth| document class is based.
\item[\href{https://www.ctan.org/pkg/multirow}{multirow}] Allows table elements to span several rows.
\item[\href{https://www.ctan.org/pkg/pgfplots}{pgfplots}] Function plot drawings.
\item[\href{https://www.ctan.org/pkg/pgf}{pgf/TikZ}] Creating graphics inside \LaTeX\ documents.
\item[\href{https://www.ctan.org/pkg/subcaption}{subcaption}] Allows the use of subfigures and enables their referencing.
\item[\href{https://www.ctan.org/tex-archive/info/symbols/comprehensive/}{symbols/comprehensive}] A listing of around 5000 symbols that can be used with \LaTeX.
\item[\href{https://www.ctan.org/pkg/voss-mathmode}{voss-mathmode}] A comprehensive overview of typesetting mathematics in \LaTeX.
\item[\href{https://www.ctan.org/pkg/xcolor}{xcolor}] Allows the definition and use of colors.
\end{description}

==> tikz/tikzEntropy.tex <==
\begin{center}
    \fbox{
    \begin{minipage}{0.45\textwidth}
        \begin{tikzpicture}[rn/.style={circle, draw=black!60, fill=lightgray!5, very thick, minimum size=8mm},]
            \node[rn, align=center]    (l-m-1)   {$\frac{1}{2}$};
            \node[rn, align=center, fill = gray]   [below left=of l-m-1]    (l-l)      {$1$};
            \node[rn, align=centerr, fill = lightgray]    (l-m-2)   [below right=of l-l]   {$\frac{1}{2}$};
            
            \draw[->, thick] (l-l.north east) to (l-m-1.west)
            \draw[->, thick] (l-l.south east) to (l-m-2.west)
        \end{tikzpicture}
    \end{minipage}
    \begin{minipage}{0.45\textwidth}
        \begin{tikzpicture}[rn/.style={circle, draw=black!60, fill=lightgray!5, very thick, minimum size=8mm},]
            \node[rn, align=center, fill = gray]      (r-l)      {$1$};
            \node[rn, align=center]    (r-m-1)   [above right=of r-l]   {$\frac{1}{2}$};
            \node[rn, align=center, fill = lightgray]    (r-m-2)   [below right=of r-l]   {$\frac{1}{3}$};
            \node[rn, align=center, fill = lightgray]    (r-m-3)   [below=of r-m-2]   {$\frac{1}{6}$};
            
            \node[rn, align=center]    (r-r-2)    [right=of r-m-1]    {$\frac{1}{4}$}
            \node[rn, align=center]    (r-r-1)    [above=of r-r-2]    {$\frac{1}{4}$}
            \node[rn, align=center, fill = lightgray]    (r-r-3)    [below=of r-r-2]    {$\frac{1}{4}$}
            \node[rn, align=center, fill = lightgray]    (r-r-4)    [below=of r-r-3]    {$\frac{1}{4}$}
            \node[rn, align=center, fill = lightgray]    (r-r-5)    [below right=of r-r-4]    {$\frac{1}{4}$}
            
            \draw[->, thick] (r-l.north east) to (r-m-1.west)
            \draw[->, thick] (r-l.south east) to (r-m-2.west)
            \draw[->, thick] (r-l.south) to (r-m-3.west)
        \end{tikzpicture}
    \end{minipage}
    }
\end{center}

